Heavy Quark Effective Theory computation of the mass of the bottom quark

We present a fully non-perturbative computation of the mass of the b-quark in the quenched approximation. Our strategy starts from the matching of HQET to QCD in a finite volume and finally relates the quark mass to the spin averaged mass of the Bs meson in HQET. All steps include the terms of order Lambda^2/Mb. Expanding on [1], we discuss the computation and renormalization of correlation functions at order 1/Mb. With the strange quark mass fixed from the Kaon mass and the QCD scale set through r0=0.5 fm, we obtain a renormalization group invariant mass Mb = 6.758(86) GeV or mb(mb)= 4.347(48) GeV in the MS-bar scheme. The uncertainty in the computed Lambda^2/Mb terms contributes little to the total error and Lambda^3/Mb^2 terms are negligible. The strategy is promising for full QCD as well as for other B-physics observables.

==> lattices.tex <==

\newcommand{\bla}{\cbla}
\newcommand{\red}{\cred}
\newcommand{\gre}{\cgre}
\newcommand{\blu}{\cblu}
\newcommand{\asylat}[1]  % \unitlength 1mm for 8 cm lattice!
{\begin{picture}(160,160)
\unitlength #1
\linethickness{0.1mm}
\blu\multiput(0,0)(0,10.0){8}{\line( 1, 0){80.0}}
\blu\multiput(0,0)(2.5,0){32}{\line( 0, 1){80.0}}
\end{picture}
}
\newcommand{\vbiglat}[1]  % \unitlength 1mm for 16 cm lattice!
{\begin{picture}(160,160)
\unitlength #1
\linethickness{0.1mm}
\blu\multiput(0,0)(0,10.0){16}{\line( 1, 0){160.0}}
\blu\multiput(0,0)(10.0,0){16}{\line( 0, 1){160.0}}
\end{picture}
}
\newcommand{\vvbiglat}[1]  % \unitlength 1mm for 32 cm lattice!
{\begin{picture}(320,280)
\unitlength #1
\linethickness{0.1mm}
\blu\multiput(0,0)(0,10.0){28}{\line( 1, 0){320.0}}
\blu\multiput(0,0)(10.0,0){32}{\line( 0, 1){280.0}}
\end{picture} 
}

\newcommand{\bwave}[1]  % \unitlength 1mm for a=1 cm lattice!
{\unitlength #1
\begin{picture}(50,20)
\linethickness{0.1 mm}
\mgt \qbezier(0,0)(1.2,20)(1.9,20)     % 0,pi/2 (pi=120)
     \qbezier(1.9,20)(2.5,20)(3.75,0)     % pi/2,pi
      \qbezier(3.75,0)(4.95,-20)(5.6,-20)
      \qbezier(5.6,-20)(6.3,-20)(7.5,0)
\end{picture}
}
\newcommand{\bwavelnod}[1]  % \unitlength 1mm for a=1 cm lattice!
{\unitlength #1
\begin{picture}(50,20)
\linethickness{0.7 mm}
\mgt \qbezier(0,0)(24,20)(37.5,20)     % 0,pi/2 (pi=120)
     \qbezier(37.5,20)(50,20)(75,0)     % pi/2,pi
      \qbezier(75,0)(99,-20)(112.5,-20)
      \qbezier(112.5,-20)(126,-20)(150,0)
\end{picture}
}
\newcommand{\bwaveasy}[1]  % \unitlength 1mm for a=1 cm lattice!
{\unitlength #1
\begin{picture}(50,20)
\linethickness{0.7 mm}
\mgt \qbezier(0,0)(12,20)(19,20)     % 0,pi/2 (pi=120)
     \qbezier(19,20)(25,20)(37.5,0)     % pi/2,pi
      \qbezier(37.5,0)(50,-20)(56,-20)
      \qbezier(56,-20)(69,-20)(75,0)
\end{picture}
}

\newcommand{\piwave}[1]  % \unitlength 1mm for a=1 cm lattice!
{\unitlength #1
\begin{picture}(50,20)
\linethickness{0.2 mm}
\gre \qbezier(0,0)(40,20)(70,20)      % 0,pi/2 (pi=140)
     \qbezier(70,20)(100,20)(140,0)   % pi/2,pi
      \qbezier(140,0)(170,-20)(210,-20)
      \qbezier(210,-20)(240,-20)(280,0)
\end{picture}
}
\newcommand{\pihwave}[1]  % \unitlength 1mm for a=1 cm lattice!
{\unitlength #1
\begin{picture}(50,20)
\linethickness{0.7 mm}
\gre \qbezier(0,0)(40,20)(70,20)      % 0,pi/2 (pi=140)
     \qbezier(70,20)(100,20)(140,0)   % pi/2,pi
\end{picture}
}





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

